Corpus-informed Retrieval Augmented Generation of Clarifying Questions

This study aims to develop models that generate corpus informed clarifying questions for web search, in a way that ensures the questions align with the available information in the retrieval corpus. We demonstrate the effectiveness of Retrieval Augmented Language Models (RAG) in this process, emphasising their ability to (i) jointly model the user query and retrieval corpus to pinpoint the uncertainty and ask for clarifications end-to-end and (ii) model more evidence documents, which can be used towards increasing the breadth of the questions asked. However, we observe that in current datasets search intents are largely unsupported by the corpus, which is problematic both for training and evaluation. This causes question generation models to ``hallucinate'', ie. suggest intents that are not in the corpus, which can have detrimental effects in performance. To address this, we propose dataset augmentation methods that align the ground truth clarifications with the retrieval corpus. Additionally, we explore techniques to enhance the relevance of the evidence pool during inference, but find that identifying ground truth intents within the corpus remains challenging. Our analysis suggests that this challenge is partly due to the bias of current datasets towards clarification taxonomies and calls for data that can support generating corpus-informed clarifications.

==> SIGIR-table-change.tex <==
\begin{table}[H]

\begin{tabular}{lrr}
\toprule
{} &  frequency &  avg($\Delta \vec{tok}$) \\
token  &              &             \\
\midrule
they  &           60 &       0.501 \\
it    &          196 &       0.480 \\
$[SEP]$ &          934 &       0.464 \\
?     &          873 &       0.458 \\
that  &           52 &       0.440 \\
.     &          192 &       0.424 \\
...   &     ...    &  ... \\\hline
macro-avg   &           -- &       0.185 \\
micro-avg   &           -- &       0.323 \\

\bottomrule
\end{tabular}

\caption{Average change of frequent token embeddings after zero-shot contextualization (all CAsT datasets).}
\label{table:mostchangingterms}
\end{table}

==> SIGIR-table-effect.tex <==


\begin{table*}[th!]
\begin{tabular}{llc||ll|ll|ll}
\multirowcell{2}{base-\\retriever} &  \multirow{2}{*}{variant}   & \multirowcell{2}{zero-\\shot}  & \multicolumn{2}{c}{CAsT'19}     & \multicolumn{2}{c}{CAsT'20}     & \multicolumn{2}{c}{CAsT'21}     \\
 &  &  & NDCG@3         & R@100         & NDCG@3         & R@100         & NDCG@3         & R@100         \\
\hline\hline

\multirow{4}{*}{ColBERT} & last-turn $^a$ & 
\ding{52} & 0.214          & 0.157     & 0.155          & 0.124      & 0.140     & 0.154    \\
& all-history $^b$ & 
\ding{52} & 0.190    & 0.165    & 0.150  & 0.166      & \textbf{0.237} & 0.265          \\
& \begin{tabular}[c]{@{}l@{}}ZeCo$^2$ \textit{(ours)}\end{tabular} & 
\ding{52} & 0.238 $^{b}$ & \textbf{0.216} $^{a,b,c}$ & \textbf{0.176} $^{b}$ & \textbf{0.200} $^{a,b,c}$ & 0.234 $^{a}$& \textbf{0.267}  $^{a}$ \\
& human  &  & 0.430           & 0.363          & 0.443          & 0.408           & 0.431          & 0.403         \\
\hline
\multirow{3}{*}{ConvDR~\cite{yu2021few}} & zero-shot $^c$ & 
\ding{52} & \textbf{0.247}          & 0.183     & 0.150      & 0.150      & --           & --       \\
& few-shot  & & 0.466          & 0.362      & 0.340        & 0.345       & 0.361           & 0.376       \\
& human   & & 0.461     & 0.389 & 0.422   & 0.454    & 0.548  & 0.451      \\
\hline

\end{tabular}
\caption{Effectiveness of zero-shot embedding contextualization on TREC-CAsT datasets.
Bold font indicates the best zero-shot performing model. Superscripts indicate statistically significant improvements (paired t-test, $p-value<0.05$) of $ZeCo^2$ over zero-shot models: \textit{last-turn $^a$, all-history $^b$} and \textit{ConvDR zero-shot $^c$} }
\vspace*{-0.6cm}
\label{tab:results-contextualization}
\end{table*}

==> SIGIR-table-match.tex <==

\begin{table*}[t]

\begin{tabular}{lll|r|lc|lc}
\multirow{3}{*}{Utterance}                                                                          & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Human \\ resolution\end{tabular}} & \multirow{3}{*}{$\Delta \vec{tok}$ } & \multirow{3}{*}{$\Delta$ Recall} 
&
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}closest match\\ (non-contextualized)\end{tabular}}
& 

\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}closest match\\ (contextualized)\end{tabular}}\\
&                                                                              &                                                                                                     &                       
& term & similarity
& term & similarity \\\hline\hline

\begin{tabular}[c]{@{}l@{}}what is the \\ first sign of \underline{\textbf{it}} ?\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}throat\\ cancer\end{tabular}                      & 0.52                                                                                                & +0.31                 & \begin{tabular}[c]{@{}l@{}}tell me about \\ lung \underline{\textbf{cancer}.}\end{tabular}     & 0.48       & \begin{tabular}[c]{@{}l@{}}what causes \\ throat \underline{\textbf{cancer}} ?\end{tabular}                 & 1          \\\hline
\begin{tabular}[c]{@{}l@{}}What is the role of \\ positivism in \underline{\textbf{it}}?\end{tabular}                  & sociology                                                                    & 0.44                                                                                                & +0.67                 & \begin{tabular}[c]{@{}l@{}}what is taught in \\ \underline{\textbf{sociology}} ?\end{tabular}                         & 0.55       & \begin{tabular}[c]{@{}l@{}}what is taught in \\ \underline{\textbf{sociology}} ?\end{tabular}               & 1          \\\hline

\begin{tabular}[c]{@{}l@{}}what technological \\ developments enabled \underline{\textbf{it}} ?\end{tabular}           & \begin{tabular}[c]{@{}l@{}}popular\\ music\end{tabular}                      & 0.54   & +0.42                 & \begin{tabular}[c]{@{}l@{}}... the origins of\\ popular \underline{\textbf{music}} ?\end{tabular}                     & 0.46       & \begin{tabular}[c]{@{}l@{}}... the origins of\\ popular \underline{\textbf{music}} ?\end{tabular}           & 1          \\\hline

\begin{tabular}[c]{@{}l@{}}what is the \\ evidence for \underline{\textbf{it}} ?\end{tabular}                          & \begin{tabular}[c]{@{}l@{}}bronze age\\ collapse\end{tabular}                & 0.36       & 0.00                 & \begin{tabular}[c]{@{}l@{}}tell me about the \\ bronze \underline{\textbf{age}} collapse.\end{tabular}                & 0.64       & \begin{tabular}[c]{@{}l@{}}tell me about the \\ bronze age \underline{\textbf{collapse}}.\end{tabular}    & 1          \\\hline

\begin{tabular}[c]{@{}l@{}}why did ben franklin want \underline{\textbf{it}} \\ to be the national symbol?\end{tabular} & turkeys                                                                      & 0.22                                                                                                & +0.29                 & \begin{tabular}[c]{@{}l@{}}where are \\ turkeys from \underline{\textbf{?}}\end{tabular}                              & 0.55       & \begin{tabular}[c]{@{}l@{}}where are \\ turkeys from \underline{\textbf{?}}\end{tabular}                    & 0.85       \\\hline

\begin{tabular}[c]{@{}l@{}}what is \underline{\textbf{it}} \\  about?\end{tabular} & \begin{tabular}[c]{@{}l@{}}neverending \\  story film\end{tabular}  & 0.39                                                                                                & +0.12                 & \begin{tabular}[c]{@{}l@{}}the neverending \\ story film \underline{.}\end{tabular}                               & 0.58       & \begin{tabular}[c]{@{}l@{}}the neverending \\ story film \underline{\textbf{.}}\end{tabular}                    & 0.88       \\\hline\hline
   
\end{tabular}

\caption{Examples of best term matches of anaphora terms in conversation history (before \& after query contextualization).}
\label{tab:closest-terms-conversation}
\end{table*}


==> SIGIR-table-similar.tex <==
\begin{table}[]

\begin{tabular}{l||ll}
   & $\vec{R}$ (resolution) & $\vec{Rnd}$ (random term)\\\hline\hline
  $\vec{A}_{last-turn}$ & 0.178           & 0.255       \\
 $\vec{A}_{ZeCo^2} $   & 0.372           & 0.204      
\end{tabular}
\caption{Embedding similarities between anaphoras and resolution or random terms from the conversations (CAsT '19).}
\vspace*{-0.3cm}
\label{tab:anaphora-resolution-random-similarities}
\end{table}

==> table-plength.tex <==
\begin{table*}[]

\begin{adjustbox}{width=\textwidth, center}
    \begin{tabular}{lll|rrr|rrr|rrr|rrrr}
    \toprule

     Evidence & n & length & \multicolumn{3}{c}{Term Overlap} & \multicolumn{3}{c}{Exact Match} & \multicolumn{3}{c}{Set-BERT} & \multicolumn{4}{c}{Set-BLEU} \\
     &&& Prec. & Rec. & F1 & Prec. & Rec. & F1 & Prec. & Rec. & F1& BLEU1 & BLEU2 & BLEU3 & BLEU4 \\
    \midrule
    \multicolumn{16}{c}{Collection: marco-doc-v1}\\\midrule
    MarcoD-aspgen\_bm25\_Q\_plen & 10 & 64 & 0.3284  & 0.2819  & 0.2905  & 0.0622  & 0.0571  & 0.0576  & 0.2737  & 0.2897  & 0.2787  & 0.2401  & 0.2003  & 0.1796  & 0.1673  \\
    MarcoD-aspgen\_bm25\_Q\_plen & 10 & 128 & 0.3273  & 0.2812  & 0.2888  & 0.0605  & 0.0597  & 0.0579  & 0.2799  & 0.2961  & 0.2850  & 0.2461  & 0.2046  & 0.1833  & 0.1701  \\
    MarcoD-aspgen\_bm25\_Q\_plen & 10 & 256 & 0.3213  & 0.2564  & 0.2731  & 0.0536  & 0.0485  & 0.0490  & 0.2624  & 0.2753  & 0.2661  & 0.2244  & 0.1856  & 0.1654  & 0.1538  \\\midrule
    MarcoD-aspgen\_bm25\_QF\_plen & 10 & 64 &  0.4028  & 0.3423  & 0.3534  & 0.1296  & 0.1263  & 0.1261  & 0.3302  & 0.3489  & 0.3358  & 0.2825  & 0.2375  & 0.2152  & 0.2014  \\
    MarcoD-aspgen\_bm25\_QF\_plen128 & 10 & 128 & 0.4009  & 0.3154  & 0.3368  & 0.1166  & 0.1173  & 0.1121  & 0.2789  & 0.2958  & 0.2841  & 0.2432  & 0.2075  & 0.1885  & 0.1766  \\
    MarcoD-aspgen\_bm25\_QF\_plen256 & 10 & 256 & 0.4077  & 0.3228  & 0.3439  & 0.1245  & 0.1189  & 0.1172  & 0.2809  & 0.2969  & 0.2857  & 0.2454  & 0.2102  & 0.1913  & 0.1792  \\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{Effect of increasing passage length during the generation of clarifying questions.}
\label{tab:passage-length}
\end{table*}
